On the Permanence of Backdoors in Evolving Models

Existing research on training-time attacks for deep neural networks (DNNs), such as backdoors, largely assume that models are static once trained, and hidden backdoors trained into models remain active indefinitely. In practice, models are rarely static but evolve continuously to address distribution drifts in the underlying data. This paper explores the behavior of backdoor attacks in time-varying models, whose model weights are continually updated via fine-tuning to adapt to data drifts. Our theoretical analysis shows how fine-tuning with fresh data progressively "erases" the injected backdoors, and our empirical study illustrates how quickly a time-varying model "forgets" backdoors under a variety of training and attack settings. We also show that novel fine-tuning strategies using smart learning rates can significantly accelerate backdoor forgetting. Finally, we discuss the need for new backdoor defenses that target time-varying models specifically.

==> Makefile <==
LATEX=pdflatex

BIBTEX=bibtex
BIBFILE=time-variant-backdoor.bib
PAPER=time-variant-backdoor

TEXFILES = time-variant-backdoor.tex \
						intro.tex\
						back.tex\
						setup.tex\
						theory.tex\
						basic.tex\
						defs.tex\
						attack.tex\
						datashift.tex\
						training.tex\
						appendix.tex\
						conclusion.tex\

FIGS = $(wildcard plots/*.pdf)

all:  $(PAPER).pdf

bib:
	$(BIBTEX) $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).pdf: $(TEXFILES) $(BIBFILE) $(FIGS)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out *.fdb_latexmk *.fls *.synctex.gz


==> intro.tex <==

\section{Introduction}
\label{sec:intro}

Given their dependence on large volumes of training
data~\cite{parkhi2015deep, ILSVRC15}, machine learning models, especially
deep neural networks (DNNs) are vulnerable
to data poisoning attacks. In a backdoor attack, attackers corrupt
training data in order to produce misclassifications on inputs with specific
characteristics~\cite{chen2017targeted, gu2017badnets, liu2018trojaning}.
Existing work has shown that backdoors are easy to inject and hard to detect,
and are considered the most worrisome attacks in a recent industry
survey~\cite{kumar2020adversarial}.  A number of proposed defenses detect and
mitigate backdoor attacks~\cite{gao2019strip,  finepruning, liu2019abs, tran2018spectral, wang2019neural}, but have generally fallen short when evaluated in a variety of attack settings, including transfer learning~\cite{yao2019latent}, federated
learning~\cite{pmlr-v97-bhagoji19a,bagdasaryan2020backdoor, wang2020attack, xie2019dba} and
physical attack scenarios~\cite{lin2020composite, wenger2021backdoor}.


A major shortcoming of existing work on backdoor attacks is a common
assumption that models are {\em static} and do not change over time.
Current research on backdoor attacks focuses on the injection process, 
either making the trigger more subtle~\cite{lin2020composite, wenger2021backdoor, nguyen2021wanet}
or addressing different threat models~\cite{yao2019latent, tang2020embarrassingly}.
It is often assumed that once a backdoor is injected, it will stay in the 
model permanently. However, in reality, most production ML models are continuously updated, either to incorporate more labeled data, or to adapt to evolving changes in the
targeted data distribution~\cite{kumar2020understanding,
  nahar2022collaboration}.  For example, ML models in recommendation systems,
user behavior classification, even road recognition in self-driving vehicles,
all need to deal with underlying target distributions that shift over time~\cite{retrain1}.
If a deployed model's target data distribution evolves, but the model does
not, the mismatch will produce significant drops in model normal accuracy. 
We use {\bf \tvmodels} to refer to models that are periodically updated with
new training data. 



There are multiple ways of updating \tvmodels{}, including transfer learning, 
online (incremental) learning and domain adaption~\cite{hoi2021online,
hoi2014libol, read2012batch, sahoo2018online, yoon2018lifelong}. 
In this paper, we focus on \tvmodels{} updated via fine-tuning (transfer learning), 
given it is the most basic, stable and standard way to address data distribution drifts of models. 
Fine-tuning was first proposed in transfer learning to address
data distribution drift~\cite{yosinski2014transferable, weiss2016survey}. 
Existing work has shown that fine-tuning is ineffective as a defense against backdoor attacks but can degrade 
the backdoor attack success rate to some degree~\cite{finepruning}.
Therefore, the question this paper aims to answer is: {\em for \tvmodels{} that are periodically updated via fine-tuning, 
how long can backdoors survive before they are removed or become ineffective?}

Different from previous work that simply claims fine-tuning can or cannot remove backdoors as a defense mechanism, our goal
is to give a comprehensive study to understand the backdoor survivability on \tvmodels{} and what factors may 
affect it. Understanding how long backdoors can survive is critical especially in the absence of foolproof defenses against backdoor attacks.




\para{Our Contributions.} 
In this paper, we launch a comprehensive study to understand how long backdoors can survive in \tvmodels{} periodically updated by fine-tuning. We first present an analytical study on backdoor
and model behaviors during fine-tuning. We prove need of model fine-tuning with data distribution drift
to confirm the motivation of our work. Our analytical results show that with sufficient training fine-tuning can remove the backdoor, while more training updates and larger learning rates can accelerate the forgetting process.
\fixme{Arjun: can you check this after the theory part is done?}


We then take an empirical approach to studying the survivability of backdoor attacks on \tvmodels{} with complex and realistic training dynamics,
since embedded backdoors are gradually degrading in the \tvmodels{},  until they
are ``forgotten'' and their triggers ineffective.
We define a new metric called {\bf backdoor survivability} on \tvmodels{}. We
explore the impact of poison ratio, trigger evasiveness and benign data shifts
on the backdoor survivability.
Following our analytical study, we show that well-chosen training strategies can significantly reduce the
backdoor survivability with negligible overhead. Finally, we discuss the
need of new backdoor defenses under the time-varying setting, given most existing defense
mechanisms cannot be directly adapted to the time-varying setting.


